Object shape error modelling and simulation during early design stage by morphing Gaussian Random Fields

Geometric and dimensional variations in objects are caused by inevitable uncertainties in manufacturing processes and often lead to product quality issues. Failing to model the effect object shape errors, i.e., geometric and dimensional errors of parts, early during design phase inhibits the ability to predict such quality issues; consequently leading to expensive design changes after freezing of design. State-of-Art methodologies for modelling and simulating object shape error have limited defect fidelity, data versatility, and designer centricity that prevent their effective application during early design phase. Overcoming these limitations a novel Morphing Gaussian Random Field (MGRF) methodology for object shape error modelling and simulation is presented in this paper. The MGRF methodology has (i) high defect fidelity and is capable of simulating various part defects including local and global deformations, and technological patterns; (ii) high data versatility and can effectively simulate non-ideal parts under the constraint of limited data availability and can utilise historical non-ideal part data; (iii) designer centric capabilities such as performing `what if?' analysis of practically relevant defects; and (iv) capability to generate non-ideal parts conforming to statistical form tolerance specification. The aforementioned capabilities enable MGRF methodology to accurately model and simulate the effect of object shape variations on product quality during the early design phase. This is achieved by first, modelling the spatial correlation in the deviations of the part from its design nominal using Gaussian Random Field and then, utilising the modelled spatial correlations to generate non-ideal parts by conditional simulations. Practical applications of developed MGRF methodology and its advantages are demonstrated using sport-utility-vehicle door parts.

==> caseStudy_before_thesis.tex <==
\section{Case study} \label{sec:Case1}


The automotive door inner, a sheet metal part which is a component of the door subassembly, is utilised to demonstrate the proposed non-ideal part modelling and simulation methodology. The methodology is illustrated for two scenarios (1)~for the case where measurement data is available, and (2)~for the case where no measurement data for the current part, but historical data for a similar part is available. In the first case, where measurement data of non-ideal part is available the covariance parameters are obtained by maximising the likelihood of parameters given measurement data. In the second case, where no measurement data is available and the covariance parameters are obtained through functional modelling of covariance parameters. The two scenarios are explained in detail in Sections~\ref{ssec:dataCase}~and~\ref{ssec:noDataCase}

\subsection{Non-ideal part modelling and simulation with measurement data } \label{ssec:dataCase}

\subsubsection{Input and pre-processing} \label{sssec:inputPreDataCase}
The inputs in this case are the Computer Aided Design (CAD) model of the ideal geometry of the part and measurement data. The CAD model of the part is converted to its mesh representation using Altair Hypermesh commercial software, the CAD along with its discrete meshed representation is illustrated in Fig.~\ref{fig:compoonentMeshes}. The mesh representation of the door inner consists of 75,000 mesh nodes and demonstrates the scalability of proposed methodology to large parts. 

\begin{figure}[htb] 
	\centering	
	\includegraphics[width=0.3\textwidth]{idealWithMesh.png}
	\caption{(a)~CAD geometry, (b)~mesh representation with key nodes}
	\label{fig:compoonentMeshes}
\end{figure}

The part measurement data in the form of CoP obtained from an optical 3D-surface scanner is illustrated in Fig.~\ref{fig:componentVariations}a, from which the deviation of each mesh node ($Z$) in the surface normal direction is calculated by routines available in \citep{Franciosa2018}. The colourmap of the obtained surface normal deviation is shown in Fig.~\ref{fig:componentVariations}b. 

\subsubsection{Characterisation of non-ideal part deviation}
In this case study, since no small scale variation or periodicity was observed in the measurement data, a single  Mat\'ern covariance function is used to characterise the deviation field, due to the computational advantages of the Mat\'ern covariance function compared to the squared exponential function \citep{Stein2012interpolation}. The optimum parameters $ \theta $ were found by maximising the likelihood,~\eqref{eq:margLik}, and the optimum values of the correlation length in X, Y and Z coordinate directions were estimated to be 168.73 mm, 7.74 mm, and 93.70 mm, respectively. The obtained optimum correlation lengths reflect the true deviation pattern seen in Fig.~\ref{fig:componentVariations}b, where a given deviation in X coordinate direction propagates longer compared to the deviations in Y and Z coordinate directions. 

\begin{figure}[htb] 
	\centering	
	\includegraphics[width=0.5\textwidth]{sourceDevInner.png}
	\caption{(a)~measured Cloud-of-Points, (b)~estimated part surface normal deviation}
	\label{fig:componentVariations}
\end{figure}

\subsubsection{Key points selection} \label{sssec:keyPtCase}

The key points in this paper are chosen uniformly from all the mesh nodes of the part, by finding the points of intersection of the part and its voxalised bounding box with cubic voxels of size 20 mm. The distance of 20 mm between two points is smaller than the optimum correlation lengths in X and Z coordinate directions enabling increased control on generated non-ideal part instances. The selected key mesh nodes for the part are coloured red and superimposed on the mesh representation in Fig.~\ref{fig:compoonentMeshes}b. 


\subsubsection{mGRF to generate non-ideal part representatives}
This section illustrates the simulation of both global and local deformation patterns, by manipulating the key point as described in Section~\ref{ssec:simulation}. Firstly, global deviations of the non-ideal part, which are simulated by manipulating a large number of key points according to the design intent is demonstrated. Global deviation can be variation such as twisting or bending of the a part about a given axis, which affect a large area of the part. In this case study a bending of the part about axis AA (Fig.~\ref{fig:golbalDef}a), giving rise to a maximum deviation of 3mm is simulated. The mean part shape simulating bending is found through GPR as described in Section~\ref{ssec:predVariation} by setting all key points to proportionately deviate about axis AA, with the farthest key point from axis being deviated by 3mm. A form error for profile of a surface with a magnitude of  $ \pm1 $ mm with statistical CI of 95\% is added to the mean bending shape, four generated non ideal part instances are shown in Fig.~\ref{fig:golbalDef}.
\begin{figure}[htb] 
	\centering	
	\includegraphics[width=\columnwidth]{golbalDef.png}
	\caption{Illustration of gobal non-ideal part deformation (a)~key points' setting, (b)~simulated part instances }
	\label{fig:golbalDef}
\end{figure}

Secondly, local deviations of the non-ideal part are simulated by manipulating few key nodes corresponding to the type of variation to be simulated. A local deviation can be a dent or a localised deformation of the flange where joining of two parts take place, these variations are of practical importance and need to be simulated. Here both dent and local flange variation of 3mm from the nominal is simulated by moving the key nodes within the back rectangles in Fig.~\ref{fig:localDef}a by 3mm. Following the setting of key point deviations, the mean part shape is found through GPR as described in Section~\ref{ssec:predVariation}, to which a form error for profile of a surface with a magnitude of $ \pm1 $ mm with statistical CI of 95\% is added. Various non-ideal part representatives generated under the given local deformation constraints are shown in Fig.~\ref{fig:localDef}b. 

Non-ideal part representatives conforming to GD\&T form tolerance specification of profile of a surface, with no global or local deformations can be simulated by setting all key point deviations to zero, and adding the generated scaled correlated spatial patterns, as described in Section~\ref{ssec:predVariation}, to the ideal surface. The key advantage of the proposed methodology is to precisely control the non-ideal behaviour at predetermined regions for simulation of several `what if?' scenarios during early design as illustrated above, and the automatic identification of region of influence of deviation through correlation lengths. %A comparison of the afore-simulated non-ideal part variation with state-of-art methodologies is not applicable as the aim is to simulate various non-ideal representatives rather than one true pattern reproduction
\begin{figure}[htb] 
	\centering	
	\includegraphics[width=\columnwidth]{localDef.png}
	\caption{Illustration of local non-ideal part deformation (a)~key points' setting, (b)~simulated part instances}
	\label{fig:localDef}
\end{figure}



\subsection{Non-ideal part modelling and simulation without measurement data } \label{ssec:noDataCase}

\subsubsection{Input and pre-processing} 
The inputs in this case are the CAD model of the ideal geometry of the part; and historical measurement data, CAD model of a similar part. The pre-processing is performed similar to case with measurement data as described in Section~\ref{sssec:inputPreDataCase}, parts are converted to their discrete mesh representations and surface normal deviations of the historical part is estimated.

\subsubsection{Characterisation of non-ideal part deviation and variation} \label{sssec:charNoData}
The optimum covariance parameters for the historical part deviation data are found by maximising the likelihood,~\eqref{eq:margLik}. Utilising this optimal covariance parameters from historical data we can model the functional relationship between process or material parameters and non-ideal deviations as described in Section~\ref{ssec:optimiseParam}. An illustration of this characterisation is shown in Fig.~\ref{fig:batchParam}, where 3-Dimensional Gaussian distributions are fit to the estimated correlation lengths of two batches of manufactured parts with different material composition. The estimated correlation lengths of parts clearly form two separate clusters, characterising the correlation lengths as a function of material composition of the part.

\begin{figure}[htb]
	\centering
	\includegraphics[width=0.5\textwidth]{3dGauss.png}
	\caption{Covariance function parameters characterisation}
	\label{fig:batchParam}
\end{figure}


\subsubsection{Key points selection and mGRF to generate non-ideal part representatives} 
The key points are selected in a manner similar to the case with measurement data as described in Section~\ref{sssec:keyPtCase}. The non-ideal part representatives of a part with no measurement data can be generated using the optimum correlation function parameters' distribution obtained from historical data, developed in Section~\ref{sssec:charNoData}, if the parts (i)~are geometrical similar, (ii)~have same material composition, and (iii)~are fabricated using the same manufacturing process. In addition to the above constraints the parts should also have the same orientation, enabling the transfer of correlation length parameters. The transformation is typically not necessary if the parts utilise the same coordinate system, such as in automotive manufacturing where all the parts use the body coordinate system.  

An illustration of the afore mentioned capability is shown in Fig.~\ref{fig:partIndepen}, where a local deformation scenario of a part with no measurement data is simulated using data from a similar part, i.e., the automotive door inner used  Section~\ref{ssec:dataCase}. In this paper the designer is tasked with making the appropriate transformation of the parts such that the generated non-ideal part representatives are physically meaningful. Also, the variation of a batch of parts can be simulated when the correlation length parameters are sampled from the estimated distribution (Section~\ref{sssec:charNoData}) for a given part.   
\begin{figure}[htb] 
	\centering	
	\includegraphics[width=0.45\textwidth]{partIndepen.png}
	\caption{Illustration of non-ideal part simulation with no data}
	\label{fig:partIndepen}
\end{figure}


\subsection{Limitation of existing deviation decomposition methodologies} \label{ssec:modeLimitCase}
 
Existing deviation decomposition based non-ideal part modelling methodologies such as natural mode analysis can generate modes without deviation data, but require measurement data to calibrate the mode to match a given spatial deviation pattern \citep{Yan2018}. However, since the mode shape depends on geodesic distances among the points on the surface \citep{Reuter2009a}, the mode shapes vary with geometry and meshing. The modes for two similar parts ordered in ascending order of magnitude is compared in Fig.~\ref{fig:modComp}, the mode shapes differ for each of the two parts and hence learning from one part cannot easily be transferred to the other part. This limitation exists for all mode based methodologies, limiting the utility of historical data.

\begin{figure}[htb] 
	\centering	
	\includegraphics[width=0.45\textwidth]{modComp.png}
	\caption{Illustration of dissimilarity of modes for two parts}
	\label{fig:modComp}
\end{figure}


\subsection{Validation of the methodology} \label{ssec:validaiton}
The ability of non-ideal part representatives generated by the proposed methodology to reproduce a given non-ideal  deviation pattern is demonstrated in the current section. The reproduction of a given non-ideal deviation is a function of number of key points and requires the non-ideal deviation at all key points. The mean deviation at all nodes for given key points' setting is predicted through GPR as described in Section~\ref{ssec:predVariation}. A sensitivity analysis for the prediction of true deviation with approximately 2000, 4000 and 8000 key points was conducted. The true and predicted non-ideal deviations along with the contour plot of error of prediction is plotted in Fig.~\ref{fig:trueDevPred}. The non-ideal deviation predicted with GPR resulted in a root mean square error of 0.0471~mm, 0.0392~mm and 0.0311~mm, respectively, which is very low and shows that the true manufactured part deviation can be predicted using the proposed methodology given all key point data. %The prediction from GPR tends to smooth the extreme values and discontinuities in true deviation as it shown in the Fig.~\ref{fig:trueDevPred}. 

The validation is conducted to demonstrate that, given enough key points deviation data, the predicted mean surface can estimate true manufactured part deviations. However, aim of the study is to simulate non-ideal part instances with spatial deviation patterns similar to the true manufactured part deviations which conform to GD\&T specifications, with little or no data, as demonstrated in the previous sections. 

\begin{figure*}[tb]
	\centering
	\includegraphics[width=0.9\textwidth]{trueDevPred.png}
	\caption{Model validation (a)~true deviation, (b)~predicted deviation, (c)~error in reproduction}
	\label{fig:trueDevPred}
\end{figure*}




==> pkgAndFormat.tex <==
\usepackage[a4paper,
top=1.5cm,
bottom=0.5cm,
left=1.5cm,
right=1.5cm,
headheight=0pt,
headsep=0pt,
marginparwidth=0pt,
marginparsep=0pt, % as per the warning by fancyhdr
includehead,includefoot,
heightrounded, % to avoid spurious underfull messages
%showframe 
]{geometry}
\usepackage{graphicx,amssymb,subcaption,amsmath}
\usepackage{natbib}
\usepackage[backref=page,hidelinks = true]{hyperref} 
\graphicspath{{./figures/}}

\renewcommand\thesection{\arabic{section}}
\renewcommand\thesubsection{\thesection.\arabic{subsection}}
\setcounter{secnumdepth}{3} % default value for 'report' class is "2"


% placeholder for image (https://gist.github.com/dpgettings/9635856)
\newcommand{\dummyfig}[1]{
	\centering
	\fbox{
		\begin{minipage}[c][0.20\textheight][c]{0.5\textwidth}
			\centering{#1}
		\end{minipage}
	}
}

%% to highlight a paragraph
\usepackage[framemethod=tikz,hidealllines=true,backgroundcolor=yellow,innerleftmargin=0pt,innerrightmargin=0pt,innertopmargin=0pt,innerbottommargin=0pt,leftmargin=0pt,rightmargin=0pt,skipabove=0pt,skipbelow=0pt]{mdframed}

%% for algorithms
\usepackage[ruled,lined,linesnumbered,dotocloa]{algorithm2e} 
\usepackage{enumerate}  

% for float restrictions			
\usepackage{placeins}                       
